UnSCAR: Universal, Scalable, Controllable, and Adaptable Image Restoration

Universal image restoration aims to recover clean images from arbitrary real-world degradations using a single inference model. Despite significant progress, existing all-in-one restoration networks do not scale to multiple degradations. As the number of degradations increases, training becomes unstable, models grow excessively large, and performance drops across both seen and unseen domains. In this work, we show that scaling universal restoration is fundamentally limited by interference across degradations during joint learning, leading to catastrophic task forgetting. To address this challenge, we introduce a unified inference pipeline with a multi-branch mixture-of-experts architecture that decomposes restoration knowledge across specialized task-adaptable experts. Our approach enables scalable learning (over sixteen degradations), adapts and generalizes robustly to unseen domains, and supports user-controllable restoration across degradations. Beyond achieving superior performance across benchmarks, this work establishes a new design paradigm for scalable and controllable universal image restoration.

==> figures/res_nano.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.68\linewidth]{figures/assets/nanopr.pdf}
    % \includegraphics[width=\linewidth]{figures/assets/mainfig.pdf}
    \caption{\textit{Zero-shot with Nano Banana Pro.} Prompting Nano Banana pro for image restoration against ours for under-display camera \cite{zhou2021image} images.}
    \label{fig:nanopro}
\end{figure}

==> method_backup.tex <==
\section{Method}
\label{sec:method}

% Existing all-in-one restoration models impose rigid architectural and training practices which prevent scaling them beyond just a few degradations. We improve upon the recent work of UniCoRN \cite{mandal2025unicorn} which proposed a flexible multi-branch supervised fine-tuned model with several of our key modifications, to make it more parameter efficient, generalizable and scalable. We highlight the architectural modifications in \cref{fig:overview} and describe them below. 

% \subsection{Model Architecture}
% \label{sec:archi}
% To overcome the scaling bottlenecks in current all-in-one restoration approaches, we propose a scalable generative framework designed for extensive multi-degrada-tion handling. Our framework rethinks feedback control synchronization, integrates semantic degradation perception, and introduces expert-based routing within a Mixture-of-Experts (MoE) control mechanism for efficient large-scale multi-degradation handling. While related to prior control-based approaches \cite{mandal2025unicorn}, our method systematically redesigns the architecture specifically for improved parameter efficiency, scalability and generalization. 


% \paragraph{Improved Feedback Control:} Image restoration methods feed in a degraded image ($I_d$) at the head based upon which the neural network aims to learn structural and pixel-level corrections to estimate a refined image ($I^*$), often called a \textit{maximum a-posteriori} (MAP) estimate. However, extending a foundational generative model such as Stable Diffusion \cite{} poses several challenges towards image recovery. First, the pretrained model should preserve it's original generative capabilities. Second, it should act as a self-adjusting restoration model based on the level of degradations present in the image. Third, any existing learned pairing with generation prompts such as texts or images need to be re-adjusted for the image restoration task where the input is a degraded image. Hence, without a proper feedback mechanism, the generative model can remain severely under-utilized in terms of its generative restoration capabilities. 

% UniCoRN \cite{mandal2025unicorn} uses the original bloated ControlNet architecture leading to slow inference times and poor generalization quality to unseen degradations. Due to feedback injection only happening in the decoder half of the model, the frozen generative encoder errors accumulate leading to extra strain on the corrections made by the control encoder. We alleviate this problem by adopting an improved feedback mechanism system \cite{zavadski2024controlnet} allowing both the control encoder and frozen backbone encoder to sync after each layer, and thus reducing the strain on the control encoder and making it lightweight ($\sim0.2\times$). Specifically, for every backbone encoder layer's output $\epsilon^k_b$ we forward it to the next control encoder layer $L^{k+1}_c$ and vice versa as,
% \begin{equation}
%     \epsilon^{k+1}_c = L_c^{k+1}(\epsilon_c^k + \epsilon_b^k);\,\,
%     \epsilon^{k+1}_b = L_b^{k+1}(\epsilon_c^k + \epsilon_b^k)
% \end{equation}
% We retain UniCoRN's original decoder control injection method without any special modifications. We also introduce a \textit{squeeze-and-excitation} module to prevent each task's restoration control being passed through the heavy control module which poses as a scaling bottleneck. The \textit{squeeze} module fuses the control signals ($\epsilon^t_c$) by simply averaging the active tasks (t), while the excitation module broadcasts the output from the control module using task specific MLP layers,

% \begin{equation}
%     s_c = \texttt{Average}(\epsilon^t_c); \,\, l^t_c = \texttt{MLP}^t(\texttt{control\_module}(s_c))
% \end{equation}
% % However, the . We adopt the efficient architecture of ControlNet-XS \cite{zavadski2024controlnet} to scale down the original model in terms of number of parameters and also provide early feedback from the control module for the model to correct degradations in the case of unseen and mixed degradations.
    
% \paragraph{Degradation-aware task embedding} Visual-Language Models (VLMs) are capable of reasoning about images to a great extent. However, surprisingly very few all-in-one restoration architectures take advantage of superior image reasoning capabilities of VLMs in identifying the nature of degradation present in the image. Similar to \cite{luo2023controlling,  chen2025real}, we augment the image embedder of CLIP \cite{radford2021learning} with an additional image controller head as shown in \cref{fig:overview}, leading to a content-aware contrastive loss (for clip embedding $p_{clip}$) and a degradation aware loss (for degradation embedding $p_{degra}$) as,
% \begin{equation}
%     L = L_{content}(\{p_{clip}\}) + L_{degradation}(\{p_{degra}\})
% \end{equation}
% \yujie{Why there is a loss term here in the architecture descriptions? Then why it is called an embedding method if the embeddings are used for loss functions?}
% However, prior works such as DA-CLIP \cite{luo2023controlling} employ a standard symmetric cross-entropy (InfoNCE) loss which contrasts positive (<image, degradation caption> pair) examples against negative examples (other <image, degradation caption> pairs). We find that this way of handling alignment works poorly for mixed degradations which is composed of multiple degradations \cref{fig:embedding}, since they can have similarity to multiple text degradation captions for the same image. Hence, we adopt SigLIP \cite{zhai2023sigmoid} loss to treat each <image, degradation caption> pair independently,
% \begin{equation}
%     -\frac{1}{|\mathcal{B}|} \sum_{i=1}^{|\mathcal{B}|} \sum_{j=1}^{|\mathcal{B}|} \log \underbrace{\frac{1}{1 + e^{z_{ij}(-t\mathbf{x}_i \cdot \mathbf{y}_j + b)}}}_{\mathcal{L}_{ij}}
% \end{equation}
% where, $\mathcal{B}$ denotes the batch size, $i$ and $j$ denote the image and caption indices, and $x$ and $y$ being the image and text features respectively. We extend the domain of the target label $z_{ij}$ to be in [0, 1] compared to the standard binary labels version, to account for mixed restoration cases. More details are included in the supplementary.

% We also scale the existing framework to distinguish between 16 unique degradation types and 9 mixed real mixed degradation types as shown in \cref{fig:embedding}, the largest degradation set ever attempted before. By utilizing degradation aware image embeddings we provide our restoration model with identifying information about different types of degradations present in the image and also provide zero-shot reasoning capabilities about degradations never seen before. 

% \input{figures/fig_daclip}

% \paragraph{Scaling mixture-of-experts (MoE) blocks} MoEs have provided a pathway for scaling large-language model performance beyond using denser transformers to parameter efficient models under tight training budgets \cite{krajewski2024scaling}. While the MoE blocks used in UniCoRN are lightweight and efficient, they pose a major scaling bottleneck when increasing the number of restoration tasks beyond just a few. \yujie{Why it poses a major obstacle for scaling? Please explain this in one or two sentences.} Hence, we adopt multi-head residual attentions  \cite{xinsir2024controlnetplus} to inflate the expert routers. However, naively performing attention on the full control latent poses another scaling challenge due to many tasks. We alleviate this problem by first performing 2D average pooling along the spatial dimensions before passing through each expert router ($E^r$). The router then fuses the restoration controls ($l^t_c$) using expert weights ($w^r_t$) for each task (t) based on the degradation-aware task embedding ($p_{degra}$) using a style modulation layer \cite{karras2020analyzing},
% \begin{equation}
%     \texttt{fused\_control\_signal} = \texttt{sum}(\underbrace{E^r(l^t_c; p_{degra})}_{w^r_t} * l_c^t)
% \end{equation}

% \input{figures/fig_lowlev}
% \paragraph{Unify low-level control} 
% \label{sec:unify}
% UniCoRN proposed the usage of low-level priors for generative restoration cues due to less variability of low-level priors over the full image from degradation to degradation (\cref{fig:l_sub1}). We expand the set of low-level priors as shown in \cref{fig:l_sub2} to account for the large set of restoration tasks tackled. Further, instead of having to manually select low-level cues per degradation task we simply unify all low-level cues, passed through a single encoder module and then broadcasted for every restoration task.

% \soumitri{
% \keypoint{Overall pipeline:}Given a LQ image $I \in \mathbb{R}^{H\times W\times3}$, our pipeline first estimates complementary structural priors and pseudo-restored images, expanding upon prior work \cite{mandal2025unicorn}. However, in addition to edge maps, color maps and dark channel prior-based transmission maps, we also integrate brightness channel priors, haze maps, texture descriptors, saturation, color-space statistics, shock and noise maps. As shown in \autoref{fig:lowlev}, these complementary cues provide diverse structural and physical perspectives on the input image required to be preserved during the restoration process. Our model is latent diffusion-based, using ControlNet \cite{controlnet} with SD 1.5 \cite{rombach2022high} as the underlying backbone. To leverage stronger priors for precise control over the generation process, we introduce a bi-directional feature feedback mechanism between the frozen SD and the controllable generative network 
% }

\subsection{Preliminaries: Unified Controllable Restoration}

Given a degraded image $\tilde{I}$, an image restoration process typically involves:
(1) identifying present degradations,
(2) balancing their restoration strengths, and
(3) predicting a residual restoration direction $R$ such that $I^*=\tilde{I}+R$.
\textsc{UniCoRN}~\cite{mandal2025unicorn} realizes this paradigm in a latent diffusion framework through conditioning mechanisms and control pathways for generative restoration.
It extracts task-specific low-level visual cues (e.g., edge, haze, noise maps) to identify degradations, 
uses lightweight mixture-of-experts (MoE) adapters to weight restoration strengths across the identified degradation types, 
and injects the balanced control signals into the latent space denoiser via a ControlNet-style mechanism.

\paragraph{Limitations of UniCoRN.} While effective, this design faces scalability challenges: 
1) Degradation-specific cue selection requires manually defined mappings, which become redundant as the number of degradations grows. 
2) UniCoRN employs ultra-lightweight MoE adapters to generate spatially varying weights that balance restoration signals across degradation types, and adopts curriculum learning for mixed degradations. However, as degradation types scale, expert routing becomes increasingly difficult to interpret and control, particularly under limited mixed-degradation training data.
3) Maintaining separate control generation pathways per degradation through ControlNet introduces significant parameter overhead and limits scalability.
%%
These limitations motivate our redesigned architecture for scalable and user-controllable restoration.


% % \soumitri{
% \subsection{Preliminaries: {Unified Controllable Restoration}} Restoring a degraded image $\tilde{I}$, requires three key steps,
% \begin{enumerate*}
%   \item identifying the degradations ($T$) present in the image, 
%   \item balancing the restoration intensity $\{w_t\}_1^T$ across the present degradations and,
%   \item providing a restoration direction ($R$) to the degraded image ($I^*\! = \!\tilde{I} \! + \! R$). 
% \end{enumerate*}
% \textsc{UniCoRN} \cite{mandal2025unicorn} follows the exact same recipe except that the restoration happens in the latent space ($l$) of Stable Diffusion architecture \cite{}. It proposes the usage of several low-level visual cues ($v_i(\tilde{I})$) such as edges, haze, color or noise maps, to identify degradations present in the input image and subsequently recruits mixture-of-experts adapters to balance the restoration intensity amongst the identified degradations. The balanced restoration cue is then fed into the main diffusion model's latent through the help of ControlNet \cite{} injections. The framework presents several strengths and weaknesses as we highlight below:
% \begin{itemize}
%     \item Low-level cues provide crucial distinguishing signals among different degradations as shown in \cref{fig:lowlev}. The degradation learning module thus picks up an inductive bias that remains easily generalizable due to simplicity of the low-level priors. \textsc{UniCoRN} proposed a selective mapping for low-level cues to be used for identifying each degradation task ($\{v_j(\tilde{I})\}_{j \in t(i)}$). However, such a mapping proves to be excessively redundant and intensive to compute when scaling the number of degradations beyond just a few. 
%     \item Mixture-of-experts when trained in a smart manner serves as viable alternative to costly training of dense models \cite{riquelme2021scaling}. UniCoRN proposed the usage of ultra-lightweight MoE adapters to adaptively weight ($w_t(x, y)$) the restoration signal spatially ($R(x, y)$) across the various present degradations. They employ a curriculum learning strategy to scale from single to mixed degradation training. However, mixed degradation datasets are scarce and multi-dimensional balancing weights are complex to gather insights into the underlying strategy employed by the expert routers, especially when balancing across 16 degradation types. This makes it difficult for a user to manually override or control the expert routers' black-box decisions. 
%     \item Residual restoration models \cite{liu2024residual, whang2022deblurring} operate by restoring the image in the residual space of the degraded image. Specifically, the aim is to learn ($\theta$) to estimate the ground truth residual ($R^* \!= \!I^* \!-\! \tilde{I}$) from just the degraded image ($\tilde{R} \!= \!f_{\theta}(\tilde{I})$). \textsc{UniCoRN} follows the widely popular ControlNet architecture which guides image generation using additive control signals in the latent space. While ControlNet operates using just a single control pathway, UniCoRN creates a separate control generation pathway for each degradation which is unscalable. Furthermore, ControlNet adds around 0.5B extra parameters to the base generative model immensely slowing down the inference times and increasing memory consumption. 
% \end{itemize}
% We propose several architectural modifications to UniCoRN to provide a scalable, user controllable, and adaptable image restoration model.
 
% 3-4 sentence paragraph about high-level overview of UniCoRN - where they exploited low-level visual cues for controllable image restoration. 
% "in this model, the most important modules allow for image restoration with low-level cues and controllability" - how we use these modules for scalability+generalization+universal restoration

\input{figures/fig_lowlev}

\subsection{\textsc{UnSCAR}} Our proposed architectural modifications are shown in \cref{fig:mainfig},
% which greatly extends the \textsc{UniCoRN} architecture 
which are designed to handle the largest set of degradations simultaneously, trained using disentangled degradation-embeddings. We also provide several instances of few-shot task and out-of-distribution adaptability with very minor architecture adjustments. 

\paragraph{\textbf{Disentangled Content-Degradation Guidance.}} Low-level visual cues ($\{v_i\}_{i=1}^I$) extracted from the degraded image ($\tilde{I}$) are structural priors which visually boost the degradations after stripping out most of the original image (see \cref{fig:lowlev}). Different low-level priors provide different degradation discrimination cues such as noise map boosting image noise while suppressing color artifacts while color map boosting grayscale appearance or haze map identifying image haze. This automatically helps We use double the number of low-level cues than used in UniCoRN, each of which gets encoded separately through a simple chain (n) of non-linear activation free (NAF) layers \cite{chen2022nafnet} and gets added to the original image's encoding before passing into the diffusion model (see \cref{fig:mainfig}.c). Low level cues are encoded as,
\begin{equation}
    \texttt{g} = \text{NAF}^n_0(\tilde{I}) + \sum_i \text{NAF}^n_i(v_i) 
\end{equation}
where g is the single unified guidance signal from the input image ($\tilde{I}$) for any degradation task compared to the task specific signals used for the prior model.

Secondly, as degradation diversity increases, precise task differentiation within the conditional pathway becomes essential to prevent feature interference. Without degradation-aware representations, control signals from heterogeneous tasks may overlap (such as for rain+fog \textit{vs} rain \textit{or} fog), leading to ambiguous conditional modulation and degraded restoration quality, particularly in mixed-degradation settings. To improve task differentiability, we introduce degradation-aware embeddings built upon a visual-language model (VLM) \cite{luo2023controlling}. Specifically, we augment the CLIP image encoder \cite{radford2021learning} with an additional degradation controller head, disentangling content embeddings $p_{clip}$ from the degradation embeddings $p_{degra}$ (\cref{fig:mainfig}.a). 


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{unscar_mainfig-compressed.pdf}
    \caption{Main Figure}
    \label{fig:mainfig}
\end{figure}


\paragraph{\textbf{Capacity-Efficient ControlNet.}} 
To realize capacity-efficient conditioning, we enhance the conditional pathway through control signal compression, efficient mixture-of-experts adapters and  bidirectional feedback synchronization (\cref{fig:mainfig}.b).

\paragraph{Shared Control Compression.}
As the number of degradation tasks increases, naively forwarding each task-specific (t) control signal  ($\epsilon$) through each heavy controlnet layer ($L^k$) introduces redundant computation and becomes a scalability bottleneck,
\begin{equation}
    \epsilon^{k}_{t} = L^k(\epsilon_t^{k-1}); \,\,\epsilon^0_t = \text{g}.
\end{equation}
%%
To maintain capacity-efficient conditioning, we introduce a lightweight \emph{squeeze-and-excite} mechanism that amortizes control computation across tasks. The \textit{squeeze} operation aggregates task-specific control features $\epsilon_c^t$ via averaging and
producing a shared control representation. The \textit{excitation} stage then redistributes this shared representation to each task through task-specific modulation units (TSU) \cite{mandal2025unicorn},
\begin{equation}
s^k = \texttt{Average}(\epsilon_t^{k-1}); \,\, \epsilon_t^k = \texttt{TSU}_t(L^k(s_c))
\end{equation}
%%
This design preserves task-specific modulation while avoiding repeated heavy control computation, thereby improving effective conditional capacity under constrained parameters and compute. \yujie{Please check this sentence's correctness.}

\paragraph{Scaling Mixture-of-Experts Adapter.} While many prior all-in-one restoration works employ inference time weighting to balance restoration trajectory \cite{mandal2025unicorn, unires}, our approach deviates in that we build an internal intuitive understanding of restoration control within the mixture-of-experts adapters. We adopt a capacity-efficient MoE routing mechanism similar to UniCoRN, except that we make it generate a single 1-dimensional vector of weights to balance restoration between detected degradations instead of using multi-dimensional weights. Thus, we make the MoE adapter perform the harder task of estimating a single global weight vector to balance the control signals from different tasks. To do this, we first shrink the input control signal ($\epsilon_t\downarrow_f$) using spatial average pooling (f) to compress the control latents before routing. Next, we split the shrunk control signals into tall (channel-wise) and wide (spatial-wise) matrices \cite{mandal2025unicorn} each of which goes through a series of residual attention blocks \cite{xinsir2024controlnetplus}. We project both the final vectors to a single dimensional vector of size $T$ representing the weight for each task. The weights are multiplied and passed through a softmax layer to sum up to 1. Each expert router $E^k$ is also conditioned with the disentangled degradation embeddings $p_{degra}$ via style modulation \cite{karras2020analyzing}:
\begin{equation}
    \epsilon^k_\text{fused}
    =
    \sum
    \underbrace{E^k(\epsilon_t^k\downarrow_f; p_{degra})}_{w^k_t}
    \cdot
    \epsilon_t^k.
\end{equation}
%%
This routing strategy expands effective conditional capacity without proportional increases in parameters or computation, enabling scalable multi-degradation restoration.

\paragraph{Bidirectional Feedback Synchronization.}
UniCoRN follows the original ControlNet paradigm, where feedback signals are injected only into the decoder layers of the diffusion backbone. The backbone encoder remains frozen and processes degraded inputs without intermediate correction.
%%
Under this decoder-only injection design, degradation-induced artifacts accumulate in encoder representations before any corrective modulation is applied. The decoder-side control branch must then compensate for these errors retroactively, increasing correction strain and limiting effective conditional capacity as degradation diversity grows.
%%
To alleviate this structural imbalance, we adopt a bidirectional synchronization mechanism, inspired by \cite{zavadski2024controlnet}, that enables feature exchange between the control encoder ($\leftarrow$) to the frozen backbone encoder ($\rightarrow$):
\begin{equation}
    \epsilon^{k+1}_{fused} = L_{c}^{k+1}(\epsilon_{fused}^k + \epsilon_{b}^k), \quad
    \epsilon^{k+1}_b = L_b^{k+1}(\epsilon_{fused}^k + \epsilon_b^k),
\end{equation}
where $\epsilon_b^k$ and $\epsilon_c^k$ denote backbone and control signal at layer $k$.
This early feature exchange distributes correction across the network, increasing effective conditional capacity while maintaining a lightweight control branch ($\sim 0.2\times$ less parameters).


% The original ControlNet paradigm \cite{controlnet} involves a late 
% %%
% UniCoRN \cite{mandal2025unicorn} follows the original ControlNet paradigm, where feedback signals are injected only into the decoder layers of the diffusion backbone. The backbone encoder remains frozen and processes degraded inputs without intermediate correction.
% %%
% Under this decoder-only injection design, degradation-induced artifacts accumulate in encoder representations before any corrective modulation is applied. The decoder-side control branch must then compensate for these errors retroactively, increasing correction strain and limiting effective conditional capacity as degradation diversity grows.
% %%
% To alleviate this structural imbalance, we adopt a bidirectional synchronization mechanism, inspired by \cite{zavadski2024controlnet}, that enables feature exchange between the control encoder and the frozen backbone encoder at each layer $k$:
% \begin{equation}
%     \epsilon^{k+1}_c = L_c^{k+1}(\epsilon_c^k + \epsilon_b^k), \quad
%     \epsilon^{k+1}_b = L_b^{k+1}(\epsilon_c^k + \epsilon_b^k),
% \end{equation}
% where $\epsilon_b^k$ and $\epsilon_c^k$ denote backbone and control features of layer $k$, respectively.
% This early feature fusion enables correction across the network, increasing effective conditional capacity while maintaining a lightweight control branch ($\approx 0.2\times$ less parameters).


\paragraph{\textbf{Residual VAE Refinement}}
Owing to the lossy nature of the variational autoencoder (VAE) utilized in SD 1.5, we perform a minor modification to the decoder architecture to make it suitable for image restoration unlike image generation where image hallucinations are permissible. Specifically, we forward the intermediate activations (for the degraded input image) from the VAE's encoder to the decoder half after the image correction happens within our model. The forwarded encoder activations are then subsequently alpha-blended with the decoder's up-sampled activations at each level using "zero"  residual convolutional blocks. 

\paragraph{\textbf{Controllable Restoration via Sliders}}
Controlling the image restoration process enhances model customizability for photo editing applications and provides greater transparency into its working principles, in contrast to prior black-box all-in-one restoration methods.
%%
We introduce a simple yet effective controllability mechanism in our universal restoration framework.
% \begin{enumerate}
%     \item Degradation control sliders - Control sliders provide a powerful way to control image generation as through text \cite{}, images \cite{dreambooth, } or concepts \cite{}. We provide an intuitive way to control degradation restoration through the use of intensity sliders. Specifically, we guide the mixture-of-experts controllers by re-weighting their fusion control weights $w^r_t$ with a user provided weight. To preserve the scale of latent space, we also normalize the new weights to be in $\mathcal{R}^1 \in [0, 1]$.
%     \item \textit{Image} concept sliders - We propose a novel application \textit{degradation concept restoration} where complex image degradations may not be classifiable into discrete categories and having a few paired examples of <high, neutral, low> of the specific degradation type would help adjust the model's restoration capabilities accordingly. We explore parameter efficient fine-tuning (PEFT) based method for generic image concepts \cite{conceptsliders} and use degraded images as the proxy concepts. Given a set (n<10) of paired degraded (+ve) and restored images (-ve) $\mathcal{S}=\{+, -\}_n$, we can train low-rank adapters to adjust the residual attentional blocks of the mixture-of-experts modules to learn complex degradation concepts,
%     \begin{equation}
%         W^* = W + \Delta W = W + A'.B'
%     \end{equation}
%     where $W$ corresponds to the weight matrix and $A'$ and $B'$ are low-rank matrices.
    
%     % \paragraph{Prompt-based guidance} -
%     % \item \paragraph{SD-Edit manipulation} - 
% \end{enumerate}
%%
%%
% Degradation control sliders - Control sliders provide a powerful way to control image generation as through text \cite{}, images \cite{dreambooth, } or concepts \cite{}. We provide an intuitive way to control degradation restoration through the use of intensity sliders. Specifically, we guide the mixture-of-experts controllers by re-weighting their fusion control weights $w^r_t$ with a user provided weight. To preserve the scale of latent space, we also normalize the new weights to be in $\mathcal{R}^1 \in [0, 1]$.

We associate each restoration task (e.g., deblurring, denoising, dehazing) with an independent user-controlled intensity slider. 
This design enables fine-grained control over different degradation types rather than relying on a single global restoration strength.
%%
Formally, let $w^t$ denote the fusion control weight generated by the mixture-of-expert adapter for a specific degradation type ($t \in T$). For each degradation, the user also specifies an intensity coefficient $\alpha_t \in [0,1]$.
The controlled fusion weights are computed (at each layer k) as
\begin{equation}
\tilde{w}^k_t = \frac{\alpha_t w^k_t}{\sum_{T} \alpha_t w^k_t},
\end{equation}
which ensures $\tilde{w}^k_t \in [0,1]$ and $\sum_t \tilde{w}^k_t = 1$.
%%
This task-wise re-weighting preserves the scale and stability of the latent representation while allowing continuous and independent control over each degradation dimension.

% \item \textit{Image} concept sliders - We propose a novel application \textit{degradation concept restoration} where complex image degradations may not be classifiable into discrete categories and having a few paired examples of <high, neutral, low> of the specific degradation type would help adjust the model's restoration capabilities accordingly. We explore parameter efficient fine-tuning (PEFT) based method for generic image concepts \cite{conceptsliders} and use degraded images as the proxy concepts. Given a set (n<10) of paired degraded (+ve) and restored images (-ve) $\mathcal{S}=\{+, -\}_n$, we can train low-rank adapters to adjust the residual attentional blocks of the mixture-of-experts modules to learn complex degradation concepts,
% \begin{equation}
%     W^* = W + \Delta W = W + A'.B'
% \end{equation}
% where $W$ corresponds to the weight matrix and $A'$ and $B'$ are low-rank matrices.

\subsection{Parameter-Efficient Unseen Adaptation}

\paragraph{Few-shot task Adaptation.}
% \vspace{-1cm}
\label{sec:fewshot}


\paragraph{Out-of-distribution Adaptation.}
% \vspace{-1cm}
\label{sec:ood}
While our model generalizes to unseen degradations in natural images, adapting to significantly different Out-of-domain (OOD) images (e.g., medical imaging) remains challenging.
%%
Leveraging the modular design of our architecture, we enable efficient OOD adaptation by introducing an auxiliary low-level encoder head (NAF chain) that processes degraded images alongside the unified low-level encoder described before. 
%%
For each new OOD dataset, we also duplicate a task-specific unit (TSU) similar to few-shot task adaptation case and its associated squeeze-excitation modules at each encoder layer, leaving the core mixture-of-experts blocks untouched. 
%%
This lightweight extension enables effective adaptation to challenging domains, such as medical imaging, without disrupting previously learned restoration capabilities or inducing catastrophic forgetting.

% \subsection{Training Objectives}


% \newpage

% \subsection{Model Architecture}
% \label{sec:overview}
% To overcome scalability bottlenecks in existing all-in-one restoration models, we propose a generative framework tailored for large-scale multi-degradation handling.
% %%
% Diffusion-based image restoration can be viewed as conditional image generation, where degraded inputs and auxiliary cues serve as conditioning signals, while the diffusion backbone provides strong natural image priors to guide clean image synthesis.
% %%
% Scaling to numerous and diverse degradation types therefore poses a fundamental challenge: as restoration is inherently conditional, scalability is governed by the expressive capacity of the conditioning pathway. As degradation diversity increases, the conditioning mechanism must deliver sufficient capacity and precision to effectively steer the generative prior, while maintaining parameter, computational, and memory efficiency.


% To this end, we enhance conditional modeling along three complementary dimensions:
% \textbf{(1) Capacity-Efficient Conditioning:} Expanding the expressive power of the conditional pathway through synchronized feedback and scalable expert routing, while maintaining parameter and computational efficiency;
% \textbf{(2) Conditioning Differentiability:} Strengthening degradation-aware representations to ensure precise task separation and modulation;
% \textbf{(3) Conditioning Signal Enrichment:} Unifying and expanding low-level priors to provide stable structural grounding across degradation types.



% \paragraph{\textbf{Capacity-Efficient Conditioning.}}
% To realize capacity-efficient conditioning, we enhance the conditional pathway through bidirectional feedback synchronization and scalable Mixture-of-Experts (MoE) routing.

% \paragraph{Bidirectional Feedback Synchronization.}
% UniCoRN \cite{mandal2025unicorn} follows the original ControlNet paradigm, where feedback signals are injected only into the decoder layers of the diffusion backbone. The backbone encoder remains frozen and processes degraded inputs without intermediate correction.
% %%
% Under this decoder-only injection design, degradation-induced artifacts accumulate in encoder representations before any corrective modulation is applied. The decoder-side control branch must then compensate for these errors retroactively, increasing correction strain and limiting effective conditional capacity as degradation diversity grows.
% %%
% To alleviate this structural imbalance, we adopt a bidirectional synchronization mechanism, inspired by \cite{zavadski2024controlnet}, that enables feature exchange between the control encoder and the frozen backbone encoder at each layer:
% \begin{equation}
%     \epsilon^{k+1}_c = L_c^{k+1}(\epsilon_c^k + \epsilon_b^k), \quad
%     \epsilon^{k+1}_b = L_b^{k+1}(\epsilon_c^k + \epsilon_b^k),
% \end{equation}
% where $\epsilon_b^k$ and $\epsilon_c^k$ denote backbone and control features at layer $k$.
% This early feature exchange distributes correction across the network, increasing effective conditional capacity while maintaining a lightweight control branch ($\sim 0.2\times$ less parameters).

% \paragraph{Shared Control Compression.}
% As the number of degradation tasks increases, naively forwarding each task-specific control signal through a heavy control module introduces redundant computation and becomes a scalability bottleneck. 
% %%
% To maintain capacity-efficient conditioning, we introduce a lightweight \emph{squeeze-and-excitation} mechanism that amortizes control computation across tasks. The \textit{squeeze} operation aggregates task-specific control features $\epsilon_c^t$ via averaging:
% $s_c = \texttt{Average}(\epsilon_c^t)$,
% producing a shared control representation. The \textit{excitation} stage then redistributes this shared representation to each task through task-specific modulation layers:
% \begin{equation}
%     l_c^t = \texttt{MLP}^t(\texttt{control\_module}(s_c)).
% \end{equation}
% %%
% This design preserves task-specific modulation while avoiding repeated heavy control computation, thereby improving effective conditional capacity under constrained parameters and compute. \yujie{Please check this sentence's correctness.}


% \paragraph{Scalable Expert Routing.}
% UniCoRN \cite{mandal2025unicorn} employs a task-aware Mixture-of-Experts (MoE) adapter, where task-specific control paths are weighted at each injection layer via separable convolution. While effective for a limited number of tasks, this per-injection MoE routing scales linearly with degradation diversity, leading to proportional growth in routing overhead and parameters.
% %%
% As degradation diversity increases, expanding expert capacity per task further amplifies computational and memory costs, particularly when routing operates over full-resolution control latents. This limits scalability in large-scale multi-degradation settings.

% To address this limitation, we adopt a capacity-efficient MoE routing mechanism that dynamically allocates task-specific modulation while bounding computational growth. Specifically, we first apply spatial average pooling to compress control latents before routing, thereby reducing attention complexity. Each expert router $E^r$ produces task-adaptive weights conditioned on degradation embeddings $p_{degra}$ via style modulation:
% \begin{equation}
%     \texttt{fused\_control\_signal}
%     =
%     \sum
%     \underbrace{E^r(l_c^t; p_{degra})}_{w_t^r}
%     \cdot
%     l_c^t.
% \end{equation}
% \yujie{The symbol $\texttt{fused\_control\_signal}$ should be refined.}
% %%
% This routing strategy expands effective conditional capacity without proportional increases in parameters or computation, enabling scalable multi-degradation restoration.

% \input{figures/fig_daclip}

% \paragraph{\textbf{Conditioning Differentiability.}}
% As degradation diversity increases, precise task differentiation within the conditional pathway becomes essential to prevent feature interference. Without degradation-aware representations, control signals from heterogeneous tasks may overlap, leading to ambiguous conditional modulation and degraded restoration quality, particularly in mixed-degradation settings.

% To improve task differentiability, we introduce degradation-aware embeddings built upon a visual-language model (VLM). Specifically, we augment the CLIP image encoder \cite{radford2021learning} with an additional degradation controller head, producing both content embeddings $p_{clip}$ and degradation embeddings $p_{degra}$. 
% % The training objective jointly optimizes content alignment and degradation discrimination:
% % \begin{equation}
% %     L = L_{content}(\{p_{clip}\}) + L_{degradation}(\{p_{degra}\}).
% % \end{equation}
% % %%
% % \yujie{Why there is a loss term here in the architecture descriptions? Then why it is called an embedding method if the embeddings are used for loss functions?}
% % Prior works such as DA-CLIP \cite{luo2023controlling} rely on symmetric InfoNCE losses that enforce one-to-one alignment between images and degradation captions. However, mixed degradations often share similarities with multiple degradation categories, making strict contrastive pairing suboptimal. 
% % %%
% % To better model multi-label degradation scenarios, we adopt the SigLIP loss \cite{zhai2023sigmoid}, which treats each image–caption pair independently:
% % \begin{equation}
% %     -\frac{1}{|\mathcal{B}|}
% %     \sum_{i=1}^{|\mathcal{B}|}
% %     \sum_{j=1}^{|\mathcal{B}|}
% %     \log
% %     \frac{1}{1 + e^{z_{ij}(-t\mathbf{x}_i \cdot \mathbf{y}_j + b)}}.
% % \end{equation}
% % Here $\mathcal{B}$ denotes the batch size, $i$ and $j$ denote the image and caption indices, and $\mathbf{x}$ and $\mathbf{y}$ being the image and text features respectively. $z_{ij} \in [0,1]$ allows soft supervision to account for mixed degradation compositions.
% % %%
% % By strengthening degradation-aware representations, our model achieves clearer task separation, more precise conditional modulation, and improved robustness to unseen or mixed degradation combinations.
% \yujie{@Deb, I've moved loss terms here to the objective section. Still need some clarifications regarding the roles of the embeddings. Please just describe how the embeddings are calculated and fed into the condition network.}

% \input{figures/fig_lowlev}
% \paragraph{\textbf{Conditioning Signal Enrichment.}}
% While capacity-efficient conditioning and task differentiation enhance the conditional pathway, scalable restoration also requires stable structural grounding. Low-level physical cues provide degradation-agnostic priors that reduce over-reliance on semantic routing.
% %%
% UniCoRN employs a limited set of low-level signals (e.g., edge and noise maps) as auxiliary guidance (Fig.~\ref{fig:lowlev}(a)). Although effective for a small number of degradation types, such cues capture only partial structural information and may be insufficient under diverse and mixed degradations.

% To enhance conditional signal richness, we significantly expand the set of low-level priors (Fig.~\ref{fig:lowlev}(b)), incorporating brightness channel priors, haze-related maps, texture descriptors, saturation cues, and color-space statistics. These complementary cues provide diverse structural and physical perspectives on the input image.
% %%
% Moreover, rather than manually selecting low-level prior sets for each task, we encode all cues through a shared encoder and broadcast the resulting representation across degradation conditions. 
% %%
% Eliminating task-specific prior selection reduces architectural branching and manual design overhead, thereby improving scalability as the number of degradation types increases. The resulting unified signal stabilizes conditional modulation and enhances robustness under diverse and mixed degradations.
% \yujie{@Deb, Check the correctness of the descriptions.}


\subsection{Training Objectives and Strategy}
\label{sec:optim}
During training, we adopt a training objective that enforces reconstruction fidelity and condition embedding supervision, and a routing stabilization strategy that stabilizes expert specialization.

\input{figures/fig_daclip}
\paragraph{\textbf{Training Objectives.}}
The overall objective is defined as,
\begin{equation}
    \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{diff}} + \lambda_{\text{pixel}} \mathcal{L}_{\text{pixel}},
\end{equation}
where $\mathcal{L}_{\text{diff}}$ is the diffusion training objective, following the DDIM formualtion~\cite{song2020denoising} with $\epsilon$-parameterization:
\begin{equation}
    \mathcal{L}_{\text{diff}}
    =
    \mathbb{E}_{t, \epsilon}
    \left[
    \| \epsilon - \epsilon_\theta(x_t, t) \|^2
    \right],
\end{equation}
where $\epsilon \sim \mathcal{N}(0,1)$ denotes Gaussian noise, $x_t$ is the noisy latent at timestep $t$, and $\epsilon_\theta(x_t,t)$ predicts the noise. $\mathcal{L}_\text{pixel}$ is a \emph{Pixel-Space Reconstruction Loss}, which is introduced to mitigate hallucinated textures and structural artifacts. $\mathcal{L}_\text{pixel}$ is defined as:
\begin{equation}
    \mathcal{L}_{\text{pixel}} = w_1\| x_\text{gt} - \mathcal{D_\phi}(\hat{z}_0) \|_1 + w_2\mathcal{L}_\texttt{SSIM} (x_\text{gt}, \mathcal{D_\phi}(\hat{z}_0)) + w_3\mathcal{L}_\texttt{LPIPS} (x_\text{gt}, \mathcal{D_\phi}(\hat{z}_0)),
\end{equation}
where $x_\text{gt}$ is the ground-truth image, $\mathcal{D_\phi}$ denotes the VAE decoder with encoder skip-connections, and $\hat{z}_0$ is the predicted clean latent from noise ($\epsilon(x_t, t)$) at time step t. $\lambda_{\text{pixel}}$ and $\lambda_{\text{cond}}$ are balancing weights.

\paragraph{Condition Embedding Supervision.}
To enable accurate degradation discrimination and task-aware routing, we supervise condition embeddings via
\begin{equation}
    \mathcal{L}_{\text{cond}} = \mathcal{L}_{\text{content}}(p_{clip})  + \mathcal{L}_{\text{degradation}}(p_{degra}).
\end{equation}
$p_{clip}$ and $p_{degra}$ denote content and degradation embeddings respectively. \yujie{@Deb, Please explain $\mathcal{L}_\text{content}$ and $\mathcal{L}_\text{degradation}$ here.}
Prior works such as DA-CLIP~\cite{luo2023controlling} rely on symmetric InfoNCE objectives \cite{radford2021learning} for both content ($\mathcal{L}_{\text{content}}$) and degradation ($\mathcal{L}_{\text{degradation}}$)  that enforce strict one-to-one alignment between images and degradation captions. However, mixed degradations often share similarities across multiple categories, making hard contrastive pairing suboptimal. 
%%
We therefore adopt the SigLIP ~\cite{zhai2023sigmoid} for the degradation loss, which models each image–caption pair independently using sigmoid activation:
\begin{equation}
    -\frac{1}{|\mathcal{B}|}
    \sum_{i=1}^{|\mathcal{B}|}
    \sum_{j=1}^{|\mathcal{B}|}
    \log
    \frac{1}{1 + e^{z_{ij}(-t\mathbf{x}_i \cdot \mathbf{y}_j + b)}},
\end{equation}
where $|\mathcal{B}|$ denotes the batch size, 
$\mathbf{x}_i$ and $\mathbf{y}_j$ are image and text features, and 
$z_{ij} \in [0,1]$ enables soft supervision for mixed degradation compositions.

\paragraph{\textbf{Expert Routers Stabilization Strategy.}}
To prevent the expert routers from converging to suboptimal local minima or collapsing into a premature ``winner-takes-all'' regime, we adopt a two-stage curriculum strategy with label smoothing. Instead of training with hard routing targets, we introduce controlled entropy into the routing target distribution.
%%
In the initial exploration phase, we allocate $\alpha \approx 0.8$ probability mass uniformly across task-relevant experts and distribute the remaining $(1-\alpha)$ mass over suboptimal experts. This relatively high-entropy target maintains gradient flow through all routing paths, mitigating dead-expert collapse and encouraging robust specialization.
%%
In the second-stage fine-tuning phase, we increase the target mass assigned to optimal experts to $0.95$, thereby reducing target entropy and promoting sparse, confident routing decisions. This curriculum progressively transitions the router from exploratory soft assignment to stable task-discriminative expert selection.
%%
Additional implementation details are provided in the supplementary material.


% \paragraph{Residual Refinement} 
% % \vspace{-1cm}
% \label{sec:refinement} 

% \subsection{Training Objectives and Strategy} 
% \label{sec:optim}
% We follow the training formulation of DDIM \cite{song2020denoising}, with $\epsilon$-parameterization as,
% \begin{equation}
%     \mathcal{L} = \mathbb{E}_{t, \epsilon} \left[ \| \epsilon - \epsilon_\theta(x_t, t) \|^2 \right]
% \end{equation}

% \noindent where $\mathcal{L}$ is the simple mean squared error loss, $\epsilon \sim \mathcal{N}(0, 1)$ denotes the ground truth Gaussian noise, $x_t$ represents the noisy input at time step $t$, and $\epsilon_\theta(x_t, t)$ is the model's prediction of that noise given the input and current time step. However, due to the generated content often exhibiting hallucinated textures such as jumbled text, malformed human hands and faces we also incorporate a pixel space loss along with the latent space diffusion loss.
% \begin{equation}
%     \mathcal{L}_{\text{pixel}} = \| x - \mathcal{D}(\hat{z}_0) \|_1
% \end{equation}

% \noindent where $x$ represents the ground truth reference image, $\mathcal{D}$ denotes the decoder (VAE) that projects the predicted clean latent $\hat{z}_0$ back into pixel space, and $\| \cdot \|_1$ is the $L_1$ norm used to enforce reconstruction fidelity and reduce artifacts.

% \paragraph{Robust Expert Selection:} To prevent the expert routers from converging to suboptimal local minima or collapsing into a ``winner-takes-all" dynamic early in training, we employ a two-stage curriculum learning strategy with label smoothing. Rather than training against hard targets, we introduce a controlled noise distribution to the expert selection ground truth. In the initial Exploration Phase, we assign $\alpha\,(\approx0.8)$ of the probability mass uniformly to the optimal experts (task-specific) and distribute remaining ($1-\alpha$) uniformly across the sub-optimal experts. This relatively high-entropy target prevents "dead experts" by ensuring gradients flow through all paths, fostering robust feature learning. During a second-stage finetuning step, we increase the target mass on the optimal experts to $0.95$. This reduction in label noise forces the router to suppress incorrect pathways and converge towards a sparser, more confident selection mechanism, effectively bridging the gap between explorative and the hard-routing behavior. More details have been included in the supplemantary.



% \subsection{Controllable Image Restoration} 
% \label{sec:infer}
% % Controlling the image restoration process makes the model more customizable for photo editing applications and provides more transparency into it's working principles unlike prior black box all-in-one restoration methods. We incorporate controllability in various forms for our universal restoration models as described below:
% Controlling the image restoration process enhances model customizability for photo editing applications and provides greater transparency into its working principles, in contrast to prior black-box all-in-one restoration methods.
% %%
% We introduce a simple yet effective controllability mechanism in our universal restoration framework.
% % \begin{enumerate}
% %     \item Degradation control sliders - Control sliders provide a powerful way to control image generation as through text \cite{}, images \cite{dreambooth, } or concepts \cite{}. We provide an intuitive way to control degradation restoration through the use of intensity sliders. Specifically, we guide the mixture-of-experts controllers by re-weighting their fusion control weights $w^r_t$ with a user provided weight. To preserve the scale of latent space, we also normalize the new weights to be in $\mathcal{R}^1 \in [0, 1]$.
% %     \item \textit{Image} concept sliders - We propose a novel application \textit{degradation concept restoration} where complex image degradations may not be classifiable into discrete categories and having a few paired examples of <high, neutral, low> of the specific degradation type would help adjust the model's restoration capabilities accordingly. We explore parameter efficient fine-tuning (PEFT) based method for generic image concepts \cite{conceptsliders} and use degraded images as the proxy concepts. Given a set (n<10) of paired degraded (+ve) and restored images (-ve) $\mathcal{S}=\{+, -\}_n$, we can train low-rank adapters to adjust the residual attentional blocks of the mixture-of-experts modules to learn complex degradation concepts,
% %     \begin{equation}
% %         W^* = W + \Delta W = W + A'.B'
% %     \end{equation}
% %     where $W$ corresponds to the weight matrix and $A'$ and $B'$ are low-rank matrices.
    
% %     % \paragraph{Prompt-based guidance} -
% %     % \item \paragraph{SD-Edit manipulation} - 
% % \end{enumerate}
% %%
% %%
% % Degradation control sliders - Control sliders provide a powerful way to control image generation as through text \cite{}, images \cite{dreambooth, } or concepts \cite{}. We provide an intuitive way to control degradation restoration through the use of intensity sliders. Specifically, we guide the mixture-of-experts controllers by re-weighting their fusion control weights $w^r_t$ with a user provided weight. To preserve the scale of latent space, we also normalize the new weights to be in $\mathcal{R}^1 \in [0, 1]$.

% \paragraph{Task-wise Degradation Control Sliders.}
% We associate each restoration task (e.g., deblurring, denoising, dehazing) with an independent user-controlled intensity slider. 
% This design enables fine-grained control over different degradation types rather than relying on a single global restoration strength.
% %%
% Formally, let $w_r^t$ denote the fusion control weight of the $t$-th expert at timestep $r$, corresponding to a specific degradation type. \yujie{@Deb, Please explain what $t$ and $r$ mean.}
% For each degradation $r$, the user specifies an intensity coefficient $\alpha_r \in [0,1]$.
% The controlled fusion weights are computed as
% \begin{equation}
% \tilde{w}_t^r = \frac{\alpha_r w_t^r}{\sum_{k} \alpha_k w_t^k},
% \end{equation}
% which ensures $\tilde{w}_t^r \in [0,1]$ and $\sum_r \tilde{w}_t^r = 1$.
% %%
% This task-wise re-weighting preserves the scale and stability of the latent representation while allowing continuous and independent control over each degradation dimension.  \yujie{@Deb, check whether this weight re-calculation formula aligns with your implementation.}

% \item \textit{Image} concept sliders - We propose a novel application \textit{degradation concept restoration} where complex image degradations may not be classifiable into discrete categories and having a few paired examples of <high, neutral, low> of the specific degradation type would help adjust the model's restoration capabilities accordingly. We explore parameter efficient fine-tuning (PEFT) based method for generic image concepts \cite{conceptsliders} and use degraded images as the proxy concepts. Given a set (n<10) of paired degraded (+ve) and restored images (-ve) $\mathcal{S}=\{+, -\}_n$, we can train low-rank adapters to adjust the residual attentional blocks of the mixture-of-experts modules to learn complex degradation concepts,
% \begin{equation}
%     W^* = W + \Delta W = W + A'.B'
% \end{equation}
% where $W$ corresponds to the weight matrix and $A'$ and $B'$ are low-rank matrices.

% % \paragraph{Prompt-based guidance} -
% % \item \paragraph{SD-Edit manipulation} - 


% \subsection{One-step restoration} 
% \label{sec:inference} 


% \subsection{Out-of-Distribution Adaptation}
% \label{sec:ood} 
% Out-of-domain (OOD) images pose a challenge for image restoration tasks compared to unseen in-distribution restoration tasks. Hence, even though our model is capable of handling several unseen degradations for naturally restoration tasks it's performance diminishes when evaluated on challenging out-od-domain image distributions such as medical imaging datasets. However, due to our modular and flexible architecture, we can adapt our model to out-of-domain distribution datasets by introducing only a few thousand parameters (<0.001\% model size). Specifically, to encode out-of-domain images we introduce a new auxiliary encoder head 
% to feed in the degraded image in addition to the unified low-level encoder discussed in \cref{sec:unify}. In addition, we clone a task specific unit (TSU) and \textit{squeeze-excitation} modules for each encoder layer for every new OOD dataset, without disturbing the mixture-of-expert blocks or other controlnet encoder modules. Through the addition of these few modules, we notice easy generalization of our foundational image restoration for challenging medical datasets without incurring catastrophic task forgetting.

 % \vspace{-3mm}   
